Reliable Conditioning of Behavioral Cloning for Offline Reinforcement Learning

Behavioral cloning (BC) provides a straightforward solution to offline RL by mimicking offline trajectories via supervised learning. Recent advances (Chen et al., 2021; Janner et al., 2021; Emmons et al., 2021) have shown that by conditioning on desired future returns, BC can perform competitively to their value-based counterparts, while enjoying much more simplicity and training stability. While promising, we show that these methods can be unreliable, as their performance may degrade significantly when conditioned on high, out-of-distribution (ood) returns. This is crucial in practice, as we often expect the policy to perform better than the offline dataset by conditioning on an ood value. We show that this unreliability arises from both the suboptimality of training data and model architectures. We propose ConserWeightive Behavioral Cloning (CWBC), a simple and effective method for improving the reliability of conditional BC with two key components: trajectory weighting and conservative regularization. Trajectory weighting upweights the high-return trajectories to reduce the train-test gap for BC methods, while conservative regularizer encourages the policy to stay close to the data distribution for ood conditioning. We study CWBC in the context of RvS (Emmons et al., 2021) and Decision Transformers (Chen et al., 2021), and show that CWBC significantly boosts their performance on various benchmarks.

==> 06-expr.tex <==
\section{Experiments}
\label{sec:expr}

% We evaluate our proposed framework on offline RL benchmarks to understand the role of conservatism in improving out-of-distribution generalization for BC, as well as to study the effectiveness of trajectory weighting in working with low-quality datasets. Moreover, we conduct ablation analysis to investigate the interplay between weighting and conservatism, and the impact of different hyperparameters.
The goal of our experiments is two-fold: (a) evaluate \name{} against benchmark approaches for offline RL via supervised learning on standard offline RL datasets, (b) ablate and analyze the individual contributions and interplay between trajectory weighting and conservative regularization.

\subsection{Evaluation on Offline RL Benchmarks} \label{sec:benchmark}

\textbf{Methods} We apply CWBC to RvS~\cite{emmons2021rvs}, a state-of-the-art BC algorithm for offline RL. 
To obtain a thorough understanding of each component of CWBC, we consider the original RvS and a few variants:
with trajectory weighting (denoted as +W), with conservatism regularization (+C), 
or with both (+W+C).
Alternative to trajectory weighting, we consider hard filtering (+F) for comparison,  where we train the model using trajectories with top 10\% returns. We also consider combining the conservatism with hard filtering (+F+C).
When the conservatism regularizer is enabled, the objective becomes $\mathcal{L}_\text{RvS} + \alpha \cdot \mathcal{C}_\text{RvS}$ (equation~\eqref{eq:obj_rvs} and~\eqref{eq:conservatism_rvs}). When the trajectory weighting is enabled, we sample data from the transformed distribution $\TildeTau$ using Algorithm~\ref{alg:weighted_sampling}. We compare our methods against two prior BC methods: DT and BC. As a reference, we also report the results of TD3+BC~\cite{fujimoto2021minimalist}, CQL~\cite{kumar2020conservative}, and IQL~\cite{iql}, current state-of-the-art value-based methods for offline RL.
% and CQL~\cite{kumar2020conservative}. 
%, where the sequence length for RvS is $1$. 
% The RvS variants are set up similarly.

\textbf{Datasets} We consider three locomotion tasks with dense rewards from the D4RL benchmark \cite{fu2020d4rl}: \hopper, \walker and \cheetah. For each task, we consider the v2 \medium, \medreplay and \medexpert offline datasets. The \medium dataset contains $1$M samples from a policy trained to approximately $\frac{1}{3}$ the performance of an expert policy. The \medreplay dataset uses the replay buffer of a policy trained up to the performance of a \medium policy. The \medexpert dataset contains $1$M samples generated by a \medium policy and $1$M samples generated by an expert policy.

\textbf{Hyperparameters}
For trajectory weighting, we use $B=20$ and $\lambda = 0.01$, and
we set the temperature parameter $\kappa$ to be the difference between the highest return and the $90$-th percentile: $\widehat{r}^{\star} - \wh{r}_{90}$,
whose value varies across the datasets.
We apply our conservatism regularization to trajectories whose returns are above the $q=95$-th percentile return in the dataset, and perturb their RTGs as described in Section~\ref{subsec:algo_conservatism}.
We use a regularization coefficient of $\alpha=1$.
% with noise sampled from uniform distributions described in Section~\ref{subsec:algo_conservatism}.
% $\epsilon \sim \mathcal{U}[0, 3000]$ \tn{likely to change}. 
% For all the environments and datasets, we set the evaluation RTG to be the expert return,
At test time, we set the evaluation RTG to be the expert return for each environment.
% as opposed to hand picking~\cite{emmons2021rvs}.
% \qq{For the conservatism regularizer, we sample noise from ...}
The model architecture and the other hyperparamters
% such as batch size and learning rate
are identical to what were used in the original paper.  

\textbf{Training and Evaluation} We train each model for $100000$ iterations.  We report the average return over $10$ training instances with different seeds, where for each instance we run $10$ evaluation rollouts. 

% \begin{table*}[t]
%     %\renewcommand{\arraystretch}{1.2}
%     \centering
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{l || l  l  l | l  l  l  | l  l  l | l | l}
%     \toprule
%      \multirow{2}{*}{}       & \multicolumn{3}{c|}{\walker}
%             & \multicolumn{3}{c|}{\hopper}
%             & \multicolumn{3}{c|}{\cheetah} & W & Avg\\ %\hline
%             & \medium & \medreplay &\medexpert 
%             & \medium & \medreplay &\medexpert
%             & \medium & \medreplay &\medexpert \\ \midrule
%     % DT      & $71.52 \pm 3.91$ & $53.37 \pm 12.18$ & $99.81 \pm 21.29$
%     %         & $59.9 \pm 4.94$ & $56.38 \pm 20.14$ & $95.35 \pm 11.25$
%     %         & $42.54 \pm 0.6$ & $34.47 \pm 4.2$ & $87.17 \pm 2.74$  & & $66.72$ \\ 
%     % DT + R  & $70.35 \pm 4.51$ & \by{$60.53 \pm 8.89$} & \by{$108.18 \pm 0.8$}
%     %         & \by{$63.87 \pm 4.4$} & \by{$76.94 \pm 5.91$} & \by{$103.44 \pm 9.03$}
%     %         & $41.61 \pm 1.69$ & \by{$36.92 \pm 2.16$} & $85.63 \pm 1.99$ & $6$ & $71.94$\\ 
%     % DT + C & $69.87 \pm 8.48$ & \by{$64.82 \pm 5.47$} & \by{$106.07 \pm 3.0$}
%     %         & $53.96 \pm 5.24$ & \by{$63.61 \pm 15.4$} & $90.06 \pm 9.25$
%     %         & $41.84 \pm 1.39$ & \by{$34.58 \pm 2.39$} & $84.04 \pm 4.95$ & $4$ & $67.65$\\
%     % DT + R + C & $70.98 \pm 5.1$ & \by{$61.45 \pm 10.95$} & \by{$108.21 \pm 0.55$}
%     %         & $56.95 \pm 9.0$ & \by{$60.48 \pm 11.59$} & \by{$100.83 \pm 10.45$}
%     %         & $41.37 \pm 1.64$ & \by{$37.93 \pm 1.76$} & $83.74 \pm 4.33$ & 5 & $69.10$ \\
%     % \midrule
%     RvS & $73.3 \pm 5.66$ & $53.96 \pm 12.05$ & $102.22 \pm 2.27$
%             & $56.57 \pm 5.49$ & $87.7 \pm 9.68$ & $108.77 \pm 0.92$
%             & $16.16 \pm 4.45$ & $-0.37 \pm 2.66$ & $83.44 \pm 2.1$ & & $64.64$ \\
%     RvS + R & $54.54 \pm 7.66$ & \by{$61.23 \pm 14.74$} & \by{$104.12 \pm 0.54$}
%             & \by{$62.51 \pm 7.06$} & \by{$92.35 \pm 6.07$} & $108.43 \pm 1.84$
%             & $3.95 \pm 5.4$ & $-0.77 \pm 2.17$ & $69.1 \pm 3.68$ & $4$ & $61.72$ \\
%     RvS + C & $71.33 \pm 4.9$ & \by{$62.0 \pm 13.52$} & $102.09 \pm 10.15$
%             & \by{$61.0 \pm 5.34$} & \by{$91.45 \pm 3.46$} & $100.95 \pm 13.4$
%             & \by{$40.68 \pm 0.95$} & \by{$36.81 \pm 1.46$} & \by{$91.2 \pm 0.97$} & $6$ & $73.06$ \\
%     RvS + R + C & \by{$73.64 \pm 5.35$} & \by{$72.8 \pm 7.45$} & \by{$107.61 \pm 0.48$}
%             & \by{$62.93 \pm 3.63$} & \by{$87.72 \pm 4.24$} & \by{$110.0 \pm 2.8$}
%             & \by{$42.21 \pm 0.66$} & \by{$40.44 \pm 0.84$} & \by{$91.1 \pm 2.03$} & $9$ & $76.49$ \\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Comparison of the normalized return on D4RL benchmark. We use +R and +C to refer to weighting and conservatism components, respectively. The last column reports the number of datasets on which the performance is improved by the variant.
%     Results are aggregated over $10$ seeds.
%     \tn{have text that mentions our approach performs even better than RvS with cherry picking the evaluation RTG}
%     % \tn{should we have a sum column?}
%     % \qq{you can give it a shot.  you can flip the rows and columns if the table is too wide} 
%     }% and $10$ evaluation rollouts per seed. }
%     %The evaluation RTG is the expert return for all the environments and datasets. \qq{The setup is written, I felt this is repeating.}}
%     \label{table:main_results}
% \end{table*}

\begin{table*}[t]
    \centering
    \caption{Comparison of the normalized return on the D4RL benchmark. We use +W, +F, +C as shorthands for weighting, filtering and conservative regularization, respectively. We use \#wins to denote the number of datasets where the variant outperforms the original RvS. Yellow: outperforming RvS. Orange: the best among all the methods. For BC and TD3+BC, we get the numbers from~\cite{emmons2021rvs}. For IQL, we get the numbers from~\cite{iql}.
    }
    \label{table:main_results}
    \resizebox{\columnwidth}{!}{
    % \begin{tabular}{l || l  l  l | l  l  l  | l  l  l | l | l}
    \begin{tabular}{l || l l l l l l l l l l l}
    \toprule
    & RvS & RvS+W & RvS+C & RvS+W+C & RvS+F & RvS+F+C & DT & BC & TD3+BC & CQL & IQL \\ \midrule
    \walker-\medium & $73.3 \pm 5.7$ & $54.5 \pm 7.7$ & $71.3 \pm 4.9$ & \by{$73.6 \pm 5.4$} & $60.9 \pm 4.9$ & $68.2 \pm 7.1$ & $71.5 \pm 3.9$ & $75.3$ & $83.7$ & $82.9$ & $78.3$ \\
    \walker-\medreplay & $54.0 \pm 12.1$ & \by{$61.2 \pm 14.7$} & \by{$62.0 \pm 13.5$} & \by{$72.8 \pm 7.5$} & $47.1 \pm 7.7$ & $53.9 \pm 11.0$ & $53.4 \pm 12.2$ & $26.0$ & $81.8$ & $86.1$ & $73.9$ \\
    \walker-\medexpert & $102.2 \pm 2.3$ & \by{$104.1 \pm 0.5$} & $102.1 \pm 10.2$ & \by{$107.6 \pm 0.5$} & $101.7 \pm 3.3$ & \by{$105.4 \pm 0.6$} & $99.8 \pm 21.3$ & $107.5$ & $110.1$ & $109.5$ & $109.6$ \\ \midrule
    \hopper-\medium & $56.6 \pm 5.5$ & \by{$62.5 \pm 7.1$} & \by{$61.0 \pm 5.3$} & \by{$62.9 \pm 3.6$} & \by{$62.4 \pm 5.0$} & \by{$65.7 \pm 6.4$} & $59.9 \pm 4.9$ & $52.9$ & $59.3$ & $64.6$ & $66.3$ \\
    \hopper-\medreplay & $87.7 \pm 9.7$ & \by{$92.4 \pm 6.1$} & \by{$91.5 \pm 3.5$} & \by{$87.7 \pm 4.2$} & \by{$91.2 \pm 5.3$} & \by{$92.1 \pm 2.9$} & $56.4 \pm 20.1$ & $18.1$ & $60.9$ & $97.8$ & $94.7$ \\
    \hopper-\medexpert & $108.8 \pm 0.9$ & $108.4 \pm 1.8$ & $101.0 \pm 13.4$ & \by{$110.0 \pm 2.8$} & $97.5 \pm 15.0$ & $105.8 \pm 3.5$ & $95.4 \pm 11.3$ & $52.5$ & $98.0$ & $102.0$ & $91.5$ \\ \midrule
    \cheetah-\medium & $16.2 \pm 4.5$ & $4.0 \pm 5.4$ & \by{$40.7 \pm 1.0$} & \by{$42.2 \pm 0.7$} & $1.4 \pm 3.3$ & \by{$36.2 \pm 2.5$} & $42.5 \pm 0.6$ & $42.6$ & $48.3$ & $49.1$ & $47.4$ \\
    \cheetah-\medreplay & $-0.4 \pm 2.7$ & $-0.8 \pm 2.2$ & \by{$36.8 \pm 1.5$} & \by{$40.4 \pm 0.8$} & \by{$-0.1 \pm 3.5$} & \by{$35.7 \pm 2.8$} & $34.5 \pm 4.2$ & $36.6$ & $44.6$ & $47.3$ & $44.2$ \\
    \cheetah-\medexpert & $83.4 \pm 2.1$ & $69.1 \pm 3.7$ & \by{$91.2 \pm 1.0$} & \by{$91.1 \pm 2.0$} & $46.0 \pm 1.5$ & $83.2 \pm 5.0$ & $87.2 \pm 2.7$ & $55.2$ & $90.7$ & $85.8$ & $86.7$ \\
    \midrule
    \# wins & / & $4$ & $6$ & \colorbox{Orange1}{$9$} & $3$ & $5$ & / & / & / & / & / \\
    average & $64.6$ & $61.7$ & $73.1$ & \colorbox{Orange1}{$76.5$} & $56.5$ & $71.8$ & $66.73$ & $51.86$ & $75.3$ & $80.6$ & $77.0$ \\
    \bottomrule
    \end{tabular}
    }
\end{table*}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{figure/rvs.pdf}
    \caption{Performance of RvS and its varaints when conditioning on different evaluation RTGs.}
    \label{fig:eval_rvs}
\end{figure}

\textbf{Results}
% \qq{start from highlighting good things:RvS+W+C outperfroms all others; +C works for RvS, RvS+W, RvS+F; +W works too and is better than +F. For the other things you want to describe, don't go too negative and no need to go to too small details}
Table \ref{table:main_results} reports the performance of different methods we consider.
Our proposed framework CWBC with all components enabled (RvS+W+C) significantly outperforms the original RvS on $9/9$ datasets, with an average improvement of $18\%$ over RvS. RvS+W+C is also the best performing model in the table, beating all other BC baselines, as well as the hybrid value-based method TD3+BC.
Conservative regularization consistently improves the results for all choices of the base models, RvS, RvS+W, and RvS+F.
RvS+F+C that relies on hard filtering of trajectories also gains notable improvements, but lags behind RvS+W+C and seems to erode the benefits of conservatism alone in RvS+C.
Trajectory weighting on its own can have varying effects on performance, but is synergistic when combined with RvS+C leading to our best performing model in RvS+W+C.
% clearly boosts the performance of RvS in low-quality \medreplay datasets, which is consistent with our analysis.

% RvS+F+C that relies on hard filtering of trajectories also gains notable improvements, but lags behind RvS+W+C. 

% To see the effectiveness of our conservative regulazation, 


% We made a thorough comparison of these two weighting mechanisms in Section~\ref{sec:ablation_rw}.
To better understand the impact of each component, we plot the achieved returns of RvS and other variants when conditioning on different values of conditioned RTG. Figure \ref{fig:eval_rvs} shows that RvS generalizes poorly to out-of-distribution RTGs, which leads to significant performance drop when the evaluation RTG is larger than the best return in the dataset. 
% Even though weighting alone (RvS+W) does improve the best achievable performance of RvS, especially in low-quality \medreplay datasets, the performance drop phenomenon shadows the absolute performance improvements shown in Table~\ref{table:main_results}.
% RvS with weighting (RvS+W) shows improvements in \medreplay datasets, which is consistent with our analysis. By upweighting trajectories with high returns (very few in \medreplay), we reduce the model bias when conditioning on large RTGs at test time, thus achieve better performance. However, RvS+W substantially underperforms the original model in the other datasets. To understand this, we plot the performance of RvS when conditioning on different values of RTG. Figure \ref{fig:eval_rvs} shows that RvS generalizes poorly to out-of-distribution RTGs, which leads to significant performance drop when the evaluation RTG is larger than the best return in the dataset. While weighting does improve the best achievable performance of RvS, it leads to faster performance drops, resulting in worsened absolute performance in Table \ref{table:main_results}. We hypothesize that this performance crash problem was the reason why the original paper had to tune the target return for every task to achieve good results.
Figure \ref{fig:eval_rvs} illustrates the significant importance of encouraging conservatism for RvS, where RvS+C has much more stable performance, even when the evaluation RTG is $2 \times$ the expert return. By explicitly asking the model to stay close to the data distribution, we achieve better out-of-distribution generalization, and avoid the performance crash problem. This leads to absolute performance improvement of RvS+C in Table \ref{table:main_results}.
CWBC combines the best of both weighting and conservatism, which enjoys good performance when conditioning on high RTG values, as well as better generalization to large, out-of-distribution RTGs.
% This is clearly shown by Table \ref{table:main_results}, where RvS+W+C outperforms RvS in all $9$ datasets by a large margin. RvS+F+C also shows improvements over RvS, but clearly underperforms RvS+W+C.

% We emphasize that out-of-distribution generalization is crucial in practice, as it allows us to flexibly choose a large RTG during evaluation and achieve good results, without knowing a priori what conditioning RTG leads to the peak performance.

% Interestingly, as opposed to RvS, the conservative regularization only marginally improves the performance of DT. Figure \ref{fig:eval_dt} shows that DT is inherently conservative to some extent, as it does not have the performance crash problem faced by RvS, even without the conservative objective. In Section \ref{sec:dt_rvs}, we conduct ablation studies to further investigate this difference in behavior between the two models. 

\subsection{Ablation Study}

\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{figure/percent_rvs.pdf}
    \caption{Comparison of trajectory weighting and hard filtering.}
    \label{fig:percent_rvs}
\end{figure}
\textbf{Trajectory Weighting versus Filtering} \label{sec:ablation_rw}
Filtering can be considered a hard weighting mechanism, wherein the transformed distribution only has support over trajectories with returns above a certain threshold. We compare this with our proposed trajectory weighting, when used alone and when combined with conservatism regularization.
Figure~\ref{fig:percent_rvs} shows that encouraging conservatism helps both forms of weighting, as +C leads to better as well as more stable performance for RvS+F. However, in almost all datasets, RvS+W+C outperforms RvS+F+C, which agrees with our analysis in Section~\ref{subsec:algo_reweight}. While hard filtering achieves the same effect of reducing bias, it completely removes the low-return trajectories, resulting in highly increased variance. Our trajectory weighting upweights the good trajectories but aims to stay close to the original data distribution, balancing this bias-variance tradeoff. This is clearly shown in Figure~\ref{fig:percent_rvs}, where RvS+W+C has much smaller variance when conditioning on large RTGs.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{figure/tune_std.pdf}
    \caption{Performance of RvS+C with different noise standard deviations.}
    %\qq{can just display $\sigma = xxx$ for simplicity}, similarly for the text}
    \label{fig:tune_std}
\end{figure}
\textbf{How Much Conservatism Is Needed?}
An important hyperparameter of CWBC is the standard deviation $\sigma$ of the noise distribution. Intuitively, a larger $\sigma$ means we want the model to be more conservative. Figure~\ref{fig:tune_std} shows the performance of RvS+C when varying the value of $\sigma$ in the \hopper datasets. RvS with $\sigma=1000$ performs the best among the variants. Noise with small standard deviations ($\sigma=10$ and $\sigma=100$) does not help much, and the model still suffers from performance crash. 
Adding too much noise ($\sigma=10000$) does not work either, as we believe that such large ood violations are harder to balance alongside the default BC loss operation on in-distribution returns.
% and not covered well enough during the course of training, which limits the out-of-distribution generalization of the model.

% \subsubsection{Trajectory weighting versus \%BC}
% A natural question one may ask is instead of weighting, why don't we just use the high-return trajectories in the dataset to train the model and filter out the low-return trajectories. This strategy is called \%BC and was introduced in \cite{chen2021decision}, where the authors perform BC on the best $10\%$ trajectories of the dataset. This is a special form of weighting, where the transformed distribution only has support for trajectories whose returns are above a certain threshold.
% \qq{add plots}

% \subsubsection{What makes DT and RvS different?} \label{sec:dt_rvs}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.8\textwidth]{figure/rtg_avg_reward.pdf}
%     \caption{Performance of DT and RvS with different conditioning formulations.}
%     \label{fig:dt_rvs}
% \end{figure}
% The results in Section \ref{sec:benchmark} show the inherent difference in nature between DT and RvS. While DT works well when conditioning on out-of-distribution RTGs, RvS fails to generalize. This difference can come from either the difference in architectures or the difference in RTG formulations (see Equation \eqref{eq:condition_rvs}) between the two models. To gain a better understanding, we train DT with the average RTG formulation (denoted as Avg-RTG) and train RvS with the RTG formulation (denoted as RTG).

% Figure \ref{fig:dt_rvs} shows the same behavior of the two models when we change their conditioning. Therefore, we hypothesize that the difference between these models stems from the difference between Transformer and MLP, and not from their RTG formulations.



% \qq{need to rewrite this...}
% One natural question to ask is why not just filtering out those high-return trajectories and run BC methods on the subset of data? 


% \tn{analyze the importance of each component and/or the important of the specific implementation/design of each component}

% \begin{itemize}
%     \item weighting vs \% BC?
%     \item weighting helps DT in low-quality datasets
%     \item RTG vs normalized RTG?
% \end{itemize}

% \subsubsection{Sequence-level versus Step-level Noise} \label{seq:noise_analyze}

==> 06-new-expr.tex <==
\section{CWBC for RvS}
\label{sec:expr}

We first apply CWBC to RvS~\cite{emmons2021rvs}, a state-of-the-art BC algorithm for offline RL, and evaluate on various benchmarks. 
To obtain a thorough understanding of each component of CWBC, we consider the original RvS and a few variants:
with trajectory weighting (denoted as +W), with conservatism regularization (+C), 
or with both (+W+C).
When the conservatism regularizer is enabled, the objective becomes $\mathcal{L}_\text{RvS} + \alpha \cdot \mathcal{C}_\text{RvS}$ (equation~\eqref{eq:obj_rvs} and~\eqref{eq:conservatism_rvs}). When the trajectory weighting is enabled, we sample data from the transformed distribution $\TildeTau$ using Algorithm~\ref{alg:weighted_sampling}.

\subsection{Evaluation on D4RL Locomotion Benchmarks} \label{sec:benchmark}

We consider three locomotion tasks with dense rewards from the D4RL benchmark \cite{fu2020d4rl}: \hopper, \walker and \cheetah. For each task, we consider the v2 \medium, \medreplay and \medexpert offline datasets. The \medium dataset contains $1$M samples from a policy trained to approximately $\frac{1}{3}$ the performance of an expert policy. The \medreplay dataset uses the replay buffer of a policy trained up to the performance of a \medium policy. The \medexpert dataset contains $1$M samples generated by a \medium policy and $1$M samples generated by an expert policy.

\textbf{Hyperparameters}
For trajectory weighting, we use $B=20$ and $\lambda = 0.01$, and
we set the temperature parameter $\kappa$ to be the difference between the highest return and the $90$-th percentile: $\widehat{r}^{\star} - \wh{r}_{90}$,
whose value varies across the datasets.
We apply our conservatism regularization to trajectories whose returns are above the $q=95$-th percentile return in the dataset, and perturb their RTGs as described in Section~\ref{subsec:algo_conservatism}.
We use a regularization coefficient of $\alpha=1$. At test time, we set the evaluation RTG to be the expert return for each environment. The model architecture and the other hyperparamters are identical to what were used in the original paper. We provide a complete list of hyperparameters in Appendix~\ref{sec:hyper}.

\begin{table*}[t]
    \centering
    \caption{Comparison of the normalized return on the D4RL locomotion benchmark. We use +W and +C as shorthands for weighting and conservative regularization, respectively. We use \#wins to denote the number of datasets where the variant outperforms the original RvS. Yellow: outperforming RvS. Orange: the best among all the methods. For BC and TD3+BC, we get the numbers from~\cite{emmons2021rvs}. For IQL, we get the numbers from~\cite{iql}. The results are averaged over 10 seeds.
    }
    \label{table:main_results}
    \resizebox{0.9\columnwidth}{!}{
    % \begin{tabular}{l || l  l  l | l  l  l  | l  l  l | l | l}
    \begin{tabular}{l || l l l l l l l l l l l}
    \toprule
    & RvS & RvS+W & RvS+C & RvS+W+C DT & BC & TD3+BC & CQL & IQL \\ \midrule
    \walker-\medium & $73.3 \pm 5.7$ & $54.5 \pm 7.7$ & $71.3 \pm 4.9$ & \by{$73.6 \pm 5.4$} & $71.5 \pm 3.9$ & $75.3$ & $83.7$ & $82.9$ & $78.3$ \\
    \walker-\medreplay & $54.0 \pm 12.1$ & \by{$61.2 \pm 14.7$} & \by{$62.0 \pm 13.5$} & \by{$72.8 \pm 7.5$} & $53.4 \pm 12.2$ & $26.0$ & $81.8$ & $86.1$ & $73.9$ \\
    \walker-\medexpert & $102.2 \pm 2.3$ & \by{$104.1 \pm 0.5$} & $102.1 \pm 10.2$ & \by{$107.6 \pm 0.5$} & $99.8 \pm 21.3$ & $107.5$ & $110.1$ & $109.5$ & $109.6$ \\ \midrule
    \hopper-\medium & $56.6 \pm 5.5$ & \by{$62.5 \pm 7.1$} & \by{$61.0 \pm 5.3$} & \by{$62.9 \pm 3.6$} & $59.9 \pm 4.9$ & $52.9$ & $59.3$ & $64.6$ & $66.3$ \\
    \hopper-\medreplay & $87.7 \pm 9.7$ & \by{$92.4 \pm 6.1$} & \by{$91.5 \pm 3.5$} & \by{$87.7 \pm 4.2$} & $56.4 \pm 20.1$ & $18.1$ & $60.9$ & $97.8$ & $94.7$ \\
    \hopper-\medexpert & $108.8 \pm 0.9$ & $108.4 \pm 1.8$ & $101.0 \pm 13.4$ & \by{$110.0 \pm 2.8$} & $95.4 \pm 11.3$ & $52.5$ & $98.0$ & $102.0$ & $91.5$ \\ \midrule
    \cheetah-\medium & $16.2 \pm 4.5$ & $4.0 \pm 5.4$ & \by{$40.7 \pm 1.0$} & \by{$42.2 \pm 0.7$} & $42.5 \pm 0.6$ & $42.6$ & $48.3$ & $49.1$ & $47.4$ \\
    \cheetah-\medreplay & $-0.4 \pm 2.7$ & $-0.8 \pm 2.2$ & \by{$36.8 \pm 1.5$} & \by{$40.4 \pm 0.8$} & $34.5 \pm 4.2$ & $36.6$ & $44.6$ & $47.3$ & $44.2$ \\
    \cheetah-\medexpert & $83.4 \pm 2.1$ & $69.1 \pm 3.7$ & \by{$91.2 \pm 1.0$} & \by{$91.1 \pm 2.0$} &  $87.2 \pm 2.7$ & $55.2$ & $90.7$ & $85.8$ & $86.7$ \\
    \midrule
    \# wins & / & $4$ & $6$ & \colorbox{Orange1}{$9$} & / & / & / & / & / \\
    average & $64.6$ & $61.7$ & $73.1$ & \colorbox{Orange1}{$76.5$} & $66.73$ & $51.86$ & $75.3$ & $80.6$ & $77.0$ \\
    \bottomrule
    \end{tabular}
    }
\end{table*}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{figure/rvs.pdf}
    \caption{Performance of RvS and its varaints when conditioning on different evaluation RTGs.}
    \label{fig:eval_rvs}
\end{figure}

\textbf{Results}
Table \ref{table:main_results} reports the performance of different methods we consider. In addition to RvS and its variants, we compare against two prior BC methods: DT and BC, and report the performance three value-based methods: TD3+BC~\cite{fujimoto2021minimalist}, CQL~\cite{kumar2020conservative}, and IQL~\cite{iql} as a reference.
Our proposed framework CWBC with all components enabled (RvS+W+C) significantly outperforms the original RvS on $9/9$ datasets, with an average improvement of $18\%$ over RvS. RvS+W+C is also the best performing BC method in the table, and is competitive with the value-based methods.
Conservative regularization consistently improves the results for both RvS and RvS+W.
Trajectory weighting on its own can have varying effects on performance, but is synergistic when combined with RvS+C leading to our best performing model in RvS+W+C.

To better understand the impact of each component, we plot the achieved returns of RvS and other variants when conditioning on different values of conditioned RTG. Figure \ref{fig:eval_rvs} shows that RvS generalizes poorly to out-of-distribution RTGs, which leads to significant performance drop when the evaluation RTG is larger than the best return in the dataset. 
Figure \ref{fig:eval_rvs} illustrates the significant importance of encouraging conservatism for RvS, where RvS+C has much more stable performance, even when the evaluation RTG is $2 \times$ the expert return. By explicitly asking the model to stay close to the data distribution, we achieve more reliable out-of-distribution performance, and avoid the performance crash problem. This leads to absolute performance improvement of RvS+C in Table \ref{table:main_results}.
CWBC combines the best of both weighting and conservatism, which enjoys good performance when conditioning on high RTG values, as well as better robustness to large, out-of-distribution RTGs.

\subsection{Evaluation on Atari games} \label{sec:atari_benchmark}
We consider $4$ games from the Atari benchmark~\citep{bellemare2013arcade}: Breakout, Qbert, Pong, and Seaquest. Similar to~\citep{chen2021decision}, for each game, we train our method on $500000$ transitions sampled from the DQN-replay dataset, which consists of $50$ million transitions of an online DQN agent~\citep{mnih2015human}. Due to the varying performance of the DQN agent in different games, the quality of the datasets also varies. While Breakout and Pong datasets are high-quality with many expert transitions, Qbert and Seaquest datasets are highly suboptimal.
% This benchmark is challenging due to its high-dimensional visual inputs and delay between actions and rewards.

\textbf{Hyperparameters}
For trajectory weighting, we use $B = 20$ bins, $\lambda = 0.1$, and $\kappa = \wh{r}^{\star} - \wh{r}_{50}$. We apply conservative regularization with coefficient $\alpha = 0.1$ to trajectories whose returns are above $\wh{r}_{95}$. The standard deviation of the noise distribution varies across datasets, as each different games have very different return ranges. During evaluation, we set the target return to $5 \times \wh{r}^{\star}$ for Qbert and Seaquest, and to $1 \times \wh{r}^{\star}$ for Breakout and Pong.

\textbf{Results}
Table~\ref{table:atari_results} summarizes the performance of RvS and its variants. CWBC (RvS+W+C) is the best method, outperforming the original RvS by $72\%$ on average. Figure~\ref{fig:eval_rvs_atari} clearly shows the effectiveness of the conservative regularization (+C). In two low-quality datasets Qbert and Seaquest, the performance of RvS degrades quickly when conditioning on out-of-distribution RTGs. By regularizing the policy to stay close to the data distribution, we achieve a much more stable performance. The trajectory weighting component (+W) alone has varying effects on performance because of the performance crash problem, but achieves state-of-the-art when used in conjunction with conservative regularization.

It is also worth noting that in both Qbert and Seaquest, CWBC achieves returns that are much higher than the best return in the offline dataset. This shows that while conservatism encourages the policy to stay close to the data distribution, it does not prohibit extrapolation. There is always a trade-off between optimizing the original supervised objective (which presumably allows extrapolation) and the conservative objective. This is very similar to other conservative regularizations used in value-based such as CQL or TD3+BC, where there is a trade-off between learning the value function and staying close to the data distribution.

\begin{table*}[t]
    \centering
    \caption{Comparison of the normalized return~\citep{hafner2020mastering} on Atari games. The results are averaged over $3$ seeds.}
    \label{table:atari_results}
    \resizebox{0.55\columnwidth}{!}{
    \begin{tabular}{l || l l l l}
    \toprule
    & RvS & RvS+W & RvS+C & RvS+W+C \\ \midrule
    Breakout & $126.9 \pm 38.0$ & $120.1 \pm 28.43$ & \by{$163.0 \pm 50.4$} & \by{$237.3 \pm 82.1$} \\
    Qbert & $-0.4 \pm 0.2$ & $0.0 \pm 0.4$ & \by{$12.4 \pm 8.6$} & \by{$19.1 \pm 2.7$} \\
    Pong & $75.7 \pm 8.6$ & \by{$90.7 \pm 6.4$} & \by{$84.1 \pm 9.6$} & \by{$90.4 \pm 1.9$} \\
    Seaquest & $0.2 \pm 0.2$ & $-0.1 \pm 0.1$ & \by{$1.6 \pm 0.2$} & \by{$1.4 \pm 0.3$} \\
    \midrule
    \# wins & / & $1$ & $4$ & $4$ \\
    average & $50.6$ & $52.7$ & $62.3$ & $87.1$ \\
    \bottomrule
    \end{tabular}
    }
\end{table*}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{figure/atari.pdf}
    \caption{Performance of RvS and its varaints on Atari games when conditioning on different evaluation RTGs. \tn{borders of figure and legend are missing}}
    \label{fig:eval_rvs_atari}
\end{figure}

\section{CWBC for DT} \label{sec:dt}
CWBC is a generic framework that can be applied to any BC methods for offline RL. In this section, we present an instantiation of CWBC in the context of Decision Transformer (DT) \cite{chen2021decision} and evaluate its performance on D4RL locomotion tasks. There are two main differences between DT and RvS. First, DT conditions on a sequence of historical states and RTGs (as opposed to only the latest step) to generate actions, using a transformer-based model. Second, the conditioning parameters of DT are the absolute RTGs $g_t$'s rather than the average RTGs $\omega_t$'s. We apply CWBC to DT with exactly the same trajectory weighting scheme and conservatism regularization used for RvS in Section~\ref{sec:expr}. Other hyperparameters of DT are identical to those used in \cite{chen2021decision}.

\begin{table*}[t]
    %\renewcommand{\arraystretch}{1.2}
    \centering
    \caption{The normalized return on D4RL locomotion tasks of DT under the CWBC framework. The results are averaged over $10$ seeds.
    % We use +W, +F, +C to refer to weighting, filtering, and conservative regularization, respectively. We use \#wins to denote the number of datasets where the variant outperforms the original RvS.
    % \qq{1 decimal?}
    }
    \label{table:dt_results}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l || l  l  l | l  l  l  | l  l  l | c | l}
    \toprule
     \multirow{2}{*}{}       & \multicolumn{3}{c|}{\walker}
            & \multicolumn{3}{c|}{\hopper}
            & \multicolumn{3}{c|}{\cheetah} & \#wins & Avg\\ %\hline
            & \medium & \medreplay &\medexpert 
            & \medium & \medreplay &\medexpert
            & \medium & \medreplay &\medexpert \\ \midrule
    DT      & $71.5 \pm 3.9$ & $53.4 \pm 12.2$ & $99.8 \pm 21.3$
            & $59.9 \pm 4.9$ & $56.4 \pm 20.1$ & $95.4 \pm 11.3$
            & $42.5 \pm 0.6$ & $34.5 \pm 4.2$ & $87.2 \pm 2.7$  & & $66.7$ \\ 
    DT + W  & $70.4 \pm 4.5$ & \by{$60.5 \pm 8.9$} & \by{$108.2 \pm 0.8$}
            & \by{$63.9 \pm 4.4$} & \by{$76.9 \pm 5.9$} & \by{$103.4 \pm 9.0$}
            & $41.6 \pm 1.7$ & \by{$36.9 \pm 2.2$} & $85.6 \pm 2.0$ & $6$ & $71.9$\\ 
    DT + C & $69.9 \pm 8.5$ & \by{$64.8 \pm 5.5$} & \by{$106.1 \pm 3.0$}
            & $54.0 \pm 5.2$ & \by{$63.6 \pm 15.4$} & $90.1 \pm 9.3$
            & $41.8 \pm 1.4$ & \by{$34.6 \pm 2.4$} & $84.0 \pm 5.0$ & $4$ & $67.7$\\
    DT + W + C & $71.0 \pm 5.1$ & \by{$61.5 \pm 11.0$} & \by{$108.2 \pm 0.6$}
            & $57.0 \pm 9.0$ & \by{$60.5 \pm 11.6$} & \by{$100.8 \pm 10.5$}
            & $41.4 \pm 1.6$ & \by{$37.9 \pm 1.8$} & $83.7 \pm 4.3$ & $5$ & $69.1$ \\
        \bottomrule
    \end{tabular}
    }
\end{table*}

\textbf{Results}
Table~\ref{table:dt_results} reports the results. DT with trajectory weighting (DT+W) outperforms DT in $6$ out of $9$ tasks with an average improvement of $8\%$. The other two variants , DT+C and DT+W+C, perform comparably to DT. Unlike RvS, the conservative regularization does not help DT much. To understand this, we visualize the performance of DT and its variants when conditioning on different evaluation RTGs in Figure~\ref{fig:dt}. Interestingly, both DT and DT+W are much less insensitive to the conditioning RTG compared to RvS, and thus does not face the performance crash problem. Therefore, adding explicit conservatism regularization does not have significant effects there.

In other words, DT enjoys the implicit self-conservatism. We hypothesize that this comes from the transformer architecture used in DT. As the policy conditions on a sequence of both state tokens and RTG tokens to predict next action, the attention layers can choose to ignore the RTG tokens while still obtaining a good prediction loss. To test this hypothesis, we experiment with a slightly modified version of DT, where we concatenate the state and RTG at each timestep instead of treating them as separate tokens. By doing this, the model cannot ignore the RTG information in the sequence. We call this version DT-Concat. Figure~\ref{fig:dt_concat} shows that the performance of DT-Concat is strongly correlated with the conditioning RTG, and degrades quickly when the target return is out-of-distribution. This experiment confirms our hypothesis.

\begin{figure}[t]
    \centering
    % \includegraphics[width=0.9\textwidth]{figure/dt.pdf}
    \includegraphics[width=0.9\textwidth]{figure/dt_std.pdf}
    \caption{Performance of DT and its variants when conditioning on different evaluation RTGs. 
    % \qq{ylim?}
    }
    \label{fig:dt}
\end{figure}

% \begin{figure}[t]
%     \centering
%     % \includegraphics[width=0.9\textwidth]{figure/rtg_avg_reward.pdf}
%     \includegraphics[width=0.9\textwidth]{figure/rtg_avg_reward_std.pdf}
%     \caption{Performance of DT and RvS when conditioning on the absolute RTG $g_t$ or the average RTG $\omega_t$.}
%     \label{fig:rtg_vs_avg_reward}
% \end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{figure/dt_concat.pdf}
    \caption{Performance of DT when the state and RTG tokens are concatenated.}
    \label{fig:dt_concat}
\end{figure}
% To understand the source of such self-conservatism, we tried switching the conditioning variable for DT and RvS:
% conditioning DT on the average RTG $\omega_t$, and conditioning RvS on the absolute RTG $g_t$.
% % $g_t$ and $\omega_t$ for RvS and DT to see if the RTG formulation is the source of the difference in behavior.
% Figure~\ref{fig:rtg_vs_avg_reward} shows that the performance of DT and RvS is not affected by the choice of the conditioning variable.
% RvS still has the performance crash problem, and DT still generalizes well to out-of-distribution RTGs. 
% Though we do not have a conclusive understanding, we hypothesize that the difference in behavior stems from the architectural differences of these two methods. We leave this question open for future works.

==> 08-checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:conclusion}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Appendix.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We include the instructions needs to reproduce our results. See Appendix~\ref{sec:appendix}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section~\ref{sec:expr}}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See Section~\ref{sec:expr}}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See Appendix~\ref{sec:appendix}}
  \item Did you mention the license of the assets?
    \answerYes{See Appendix~\ref{sec:appendix}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{Our work does not introduce any new assets.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{The data we use is publicly available}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{The data we use is publicly available and it does not contain any personally identifiable information or offensive content.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}
\end{enumerate}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

